Simple Recursive Games

We define the class of "simple recursive games". A simple recursive game is defined as a simple stochastic game (a notion due to Anne Condon), except that we allow arbitrary real payoffs but disallow moves of chance. We study the complexity of solving simple recursive games and obtain an almost-linear time comparison-based algorithm for computing an equilibrium of such a game. The existence of a linear time comparison-based algorithm remains an open problem.

==> interdict.tex <==
We are given a network $(V,E)$ with arc capacities $c : E \to \mathbf{R}^+$, a source $s$, and a
destination $t$. From each vertex $v$ we are allowed to remove at most 
$k(v)$ outgoing
arcs,\footnote{We could, as in \cite{KhachiyanEtAl:2007}, allow more general budget constraints,
  specified by a certain class of oracles, without affecting the asymptotic
  running time of our algorithms.}
%\footnote{We can allow more general budget type constraints, where
%  we assume that each vertex has an oracle (with state) that says
%  whether a given arc can be removed within the budget (together with
%  previously removed ones),
%  and if so, removes it.}
and we seek to destroy wide paths from $s$ to $t$ (the width of
a path is the
minimum capacity along that path). As for the SRGs, we will for
simplicity assume that capacities are distinct. We also assume that
$|E| \geq |V|$.

For any vertex, $\Width(v)$ denotes the minimax width we can achieve for
paths from $v$ to $t$. If we can destroy all paths, then $\Width(v)=0$,
and we
define $\Width(t)=+\infty$.
%
As for the SRGs, the \emph{widest path interdiction} problem can be
solved weakly, which is to compute $\Width(s)$ and corresponding arcs to
remove, or strongly, which is to compute $\Width(v)$ for \emph{all} vertices
$v$ and corresponding arcs to remove. The problem is related to SRGs
as follows.
%Computing $\Width(s)$ is called the \emph{widest path interdiction} problem, and is related to
%simple recursive games as follows.
\begin{proposition}
If widest path interdiction can be weakly (resp. strongly) solved in %$O(f(|E|+|V|))$ 
linear time, then SRGs can be weakly (resp. strongly) solved in %$O(f(m+n))$ 
linear time.
\end{proposition}
\begin{proof}
Suppose that
all terminal payoffs are positive. Introduce a supersink
and connect each terminal to it by an arc with capacity equal to the
terminal payoff. Let all other arcs have capacity $+\infty$. At each
$\pn$-vertex, all but $1$ outgoing arc may be removed. At all other
vertices, no outgoing arcs may be removed.
\qed\end{proof}

\subsection{Strongly, with Sorted Capacities}

Suppose that we are also given a permutation that sorts the list of arcs by
capacity. Then we can
%find the values (and which arcs to remove) for all vertices
solve the problem strongly
in linear time
as follows.

\begin{enumerate}
\item $\Width[V] := 0$
\item $\Width[t] := +\infty$
\item While $\mbox{indeg}(t) > 0$
\begin{enumerate}
\item Let $e$ be a max-capacity incoming arc to $t$, and let $v$ be its tail.
%\item Let $v$ be the tail of $e$.
\item If $v$'s budget allows it, remove $e$ (this is an
  optimal removal).
\item Else, ensure that arcs to $v$ have capacity at most $\Width[v]:=c(e)$,
remove all outgoing arcs from $v$, and merge $v$
with $t$.
\end{enumerate}
\end{enumerate}

To implement the algorithm, we need a max-priority queue for the incoming
arcs to $t$. Fortunately,
extracted values form a non-increasing sequence, so we can first replace
the capacities with integers from $1$ to $m$ (using the given
permutation) and then use an
array of $m$ buckets to stay within linear time.

\begin{remark}
This algorithm resembles the $O(|E|\log |V|)$ algorithm in \cite{KhachiyanEtAl:2007}, which is used for \emph{shortest} paths
interdiction. However, assuming sorted arc weights does not
improve that algorithm (since not only their relative order matters). 
\end{remark}

\subsection{Weakly, with Unsorted Capacities}
%\emph{For simplicity, we will assume that all arcs in the given network
%have different capacities. This can
%easily be simulated by differentiating arcs with equal capacities in
%some arbitrary (but consistent) way.}


We keep an array $C$ of capacities, initially containing all
capacities. We repeat the following.

\begin{enumerate}
\item Partition $C$ into $2^{|E|/|C|}$
  groups of (almost) equal size.
\item Use the algorithm from the previous subsection on the coarse
  network (obtained by treating all capacities in the same group as
  equal) to find the group $C'$
  containing $\Width(s)$.
\item Replace capacities below and above $C'$ with $0$ and
  $+\infty$, respectively, and assign $C:=C'$.
\end{enumerate}
%
%If $m_i$ denotes $|C|$ after $i$ iterations, it is not hard to prove
%that $m_i \leq \frac{m}{2\uparrow\uparrow i}$ (disregarding some constants). Since each iteration
%takes $O(m)$ time, the total running time is $O(m \log^* m)$.
%
Analysis similar to that of Section \ref{logstar_analysis}
now gives the following.
%shows that the running
%time is $O(|E| \log^* |E|)$.
\begin{theorem}
The widest path interdiction problem can be weakly solved in time $O(|E|
\log^* |E|)$.
\qed
\end{theorem}
If we in step 1 replace $2^{|E|/|C|}$ with just $2$, we
instead have the following.
\begin{theorem}
The widest path interdiction problem can be weakly solved in time $O(|E|
\log\log |E|)$ and $O(|E|)$ comparisons.
\qed
\end{theorem}
%\begin{enumerate}
%\item Define SRGs. (Allow multiple terminals with the same payoff.)
%\item Define the concept of value (without asserting existence).
%\item Solve acyclic SRGs in linear time.
%\item Define merging operations.
%\item Solve ordered SRGs in linear time.
%\item Lower bound by sorting networks.
%\item Interval lemma.
%\item Log star algorithm (idea: zoom-operator $Zoom(G,k)$, pseudo-code, bounds, practical
%  considerations).
%\item Linear number of comparisons.
%\item Constructing strategies from values (all/single).
%\item Comments: What is keeping us from linear time? Cycles are not needed, but still cause problems! (Like shortest
%  paths.)
%
%\end{enumerate}
%\paragraph{Open question.} Of course, we can also construct the widest path within
%this time. Is it possible to just find a widest path (without interdiction)
%faster than this (inverse Ackermann or linear)?

%\paragraph{Open question.} When the budget is \emph{global}, e.g. we can remove any
%$k$ arcs, is the problem $\mathbf{NP}$-hard (as for shortest paths interdiction)? 

%%% Local Variables: ***
%%% mode:latex ***
%%% tex-main-file: "srg.tex"  ***
%%% TeX-master: "srg.tex" ***
%%% End: ***


==> logstar.tex <==
When weakly solving an SRG, we can balance the partitioning and
retrograde analysis to achieve an almost linear running time, by a technique
similar to the one used in \cite{GabowTarjan:1988} and later generalized
in \cite{Punnen:1996}.\footnote{Note, however, that while the
  technique
is simiilar, neither the problem of solving simple recursive games, nor the
  widest path interdiction problem of the next section, seem to fit
  into the framework of \cite{Punnen:1996}.}
As noted in section \ref{prelim}, we may assume that all vertices have positive values.

\subsection{Algorithm}
%Let $v$ be the starting vertex.
Given an SRG $G$ with $m$ arcs and $n$ terminals and starting position
$v_0$, do the following
for $i=0,1,2,\ldots$
\begin{enumerate}
\item \label{part} Partition the current set of $n_i$ terminals into
%$2^{\frac{m}{n_i}}$
%groups of equal size.
groups of size at most $\frac{n_i}{2^{\frac{m}{n_i}}}$.
%NB: No group may contain both positive and 
%negative terminals!
\item \label{solve} Solve the coarse game obtained by merging the
  terminals in each group.
\item Remove all vertices having values outside the group of $\Val_G(v_0)$. 
%(If the
%  value of $v$ was found to be $0$, then stop.)
%\item Merge groups below that of $v$ into a single terminal.
%\item Merge groups above that of $v$ info a single terminal.
\item Undo step \ref{part} for the group of $v_0$.
\label{end}
\end{enumerate}
When $\frac{n_i}{2^{\frac{m}{n_i}}} < 1$, stop and solve the remaining game by the
sorting method.
\subsection{Analysis}
\label{logstar_analysis}
All steps can be performed in $O(m+n)$ time. For the first step we can do a  ``partial perfect Quicksort'',
where we always partition around the median (which can be done in
linear time 
by Blum {\em et al} \cite{BlumFloydPrattRivestTarjan:1972}) and stop at
level $\lceil \frac{m}{n_i} \rceil +1$.

To bound the
number of iterations, we note that $n_i$ satisfies the recurrence
\begin{equation}
n_{i+1} \leq \frac{n_i}{2^{\frac{m}{n_i}}}\,,
\end{equation}
which by induction gives
\begin{equation}
n_i \leq \frac{n}{  2^{\frac{m}{n}2^{\frac{m}{n}{\rotatebox{10}{\ldots}}^{2^{\frac{m}{n}}}}}}
\hspace{-1.3cm}\raisebox{-.35cm}{\rotatebox{-75}{\Bigg\}}\hspace{-.6cm}\raisebox{-.5cm}{$i$}}
\end{equation}
Thus, the number of iterations is $O(\log^*_{2^{\frac{m}{n}}} n)$,
where $\log^*_b$ denotes the number of times we need to apply the base
$b$ logarithm function to get below $1$.
This is easily seen to be equivalent to 
$O(\log^* m - \log^* \frac{m}{n})$. 
% (PROOF NEEDED?!) I'd say no, but I now have a very easy proof:
% ONE iteration of log_{2^{m/n}} is no better than TWO iterations
% of log_2 except when the number you apply them to becomes smaller
% than, say, 2^2^{m/n}. Then, log_{2^{m/n}} makes the number
% disappear in O(1) iterations, while log has to work for another 
% O(log*(m/n)) iterations.
% This actually gives you log^* n - .. rather than log^* m
% but as we observed, we should write m to be correct also when
% n < m/n. PBM.
 We have now established the following.
\begin{theorem}
An SRG with $m$ arcs and $n$ terminals can be weakly solved in
$O(n + m + m (\log^*(m)-\log*(m/n)))$ time.\qed
% I have to add + m, as the third term might (easily) be 0
\end{theorem}

\begin{remark}
{\ }
\begin{itemize}
\item If $m = \Omega(n\log^{(k)} n)$ for some constant $k$, then
  $O(n+ m + m (\log^*(m)-\log*(m/n))) = O(m)$.
%\item If vertex values are somewhat evenly distributed, then the decrease in
%  the number of non-terminals will yield a linear running time.
% I've commented out the above. I think this statement should be made
% precise or removed. It should not be a vague remark about
%``practical'' performance, as log* is constant for all practical
% purposes anyway!
%\item $O(n+m \log^*_{2^{\frac{m}{n}}} n) \subseteq O(m+n\log\log n)$.
%\item Instead of only merging terminals, we can also merge the internal
%  vertices with the corresponding values. Provided that values are
%  distributed somewhat evenly, this will most likely give linear time performance...
\end{itemize}
\end{remark}
%%% Local Variables: ***
%%% mode:latex ***
%%% tex-main-file: "srg.tex"  ***
%%% TeX-master: "srg.tex" ***
%%% End: ***

